Computing the distance distribution of systematic non-linear codes

The most important families of non-linear codes are systematic. A brute-force check is the only known method to compute their weight distribution and distance distribution. On the other hand, it outputs also all closest word pairs in the code. In the black-box complexity model, the check is optimal among closest-pair algorithms. In this paper we provide a Groebner basis technique to compute the weight/distance distribution of any systematic non-linear code. Also our technique outputs all closest pairs. Unlike the check, our method can be extended to work on code families.

==> tables.tex <==
\subsection{Numerical computations}


We provide some numerical computations.
We have collected our results in three blocks, any containing
three consecutive tables.
The values in the first block have been obtained with the software package Magma,
those in the second block have been obtained with the software package Singular, and those in the third with the software package
 Cocoa.
In all tables, we consider codes with $n=2k$ and $d\sim (n-k)$, which is the
hardest case due to the Singleton's bound.
In the first table of any block we consider random codes with $\deg({\sf f}_i)=k$.
In the second table we consider random quadratic codes ($\deg({\sf f}_i)=2$).
In the third table we consider random linear codes ($\deg({\sf f}_i)=1$).
%manca la frase delle caratteristiche della macchina
These tests has been done on a dual AMD Opteron 2GHz, 
equipped with 8GB of RAM memory, at the computational centre MEDICIS.
\\
{\tiny

\centerline{\bf Computations with Magma}
$$
  \begin{array}{|c|c|c|}
  \hline
  n  & k & \rm{time}    \\
  \hline
  4  & 2 & < .001 s  \\
  6  & 3 & <.001 s  \\
  8  & 4 & <.001 s   \\
  10 & 5 & \sim 2.20 s  \\
  12 & 6 & \sim 264.64 s  \\         
  \hline             
  \end{array}
  \qquad
  %
  \begin{array}{|c|c|c|}
  \hline
  n  & k & \rm{time}    \\
  \hline
  4  & 2 & < .001 s  \\
  6  & 3 & <.001 s\\
  8  & 4 & <.001  s    \\
  10 & 5 & \sim 1.49 s   \\
  12 & 6 & \sim 22.73 s   \\   
  \hline
  \end{array}
  \qquad
  %
  \begin{array}{|c|c|c|}
  \hline
  n  & k & \rm{time}    \\
  \hline
  4  & 2 & < .001 s  \\
  6  & 3 & < .001 s  \\
  8  & 4 & <.001 s \\
  10 & 5 &  <.001 s  \\
  12 & 6 & \sim 3.04 s \\        
  \hline
  \end{array}
$$


%\pagebreak


\centerline{\bf Computations with Cocoa}
$$
  \begin{array}{|c|c|c|}
  \hline
  n  & k & \rm{time}    \\
  \hline
  4  & 2 & < .001 s  \\
  6  & 3 & <.001 s  \\
  8  & 4 & <.001 s   \\
  10 & 5 & \sim 32.12 s \\
  12 & 6 & > 10 h  \\         
  \hline             
  \end{array}
  \qquad
  %
  \begin{array}{|c|c|c|}
  \hline
  n  & k & \rm{time}    \\
  \hline
  4  & 2 & < .001 s  \\
  6  & 3 & <.001 s  \\
  8  & 4 & <.001 s    \\
  10 & 5 & \sim 8.65 s   \\
  12 & 6 &  \sim 4h         \\   
  \hline
  \end{array}
  \qquad
  %
  \begin{array}{|c|c|c|}
  \hline
  n  & k & \rm{time}    \\
  \hline
  4  & 2 & < .001 s  \\
  6  & 3 & < .001 s  \\
  8  & 4 & <.001s \\
  10 & 5 &  <.001 s  \\
  12 & 6 & \sim 5.04 s    \\        
  \hline
  \end{array}
$$




\centerline{\bf Computations with Singular}
$$
  \begin{array}{|c|c|c|}
  \hline
  n  & k & \rm{time}    \\
  \hline
  4  & 2 & < .001 s  \\
  6  & 3 & < .001 s  \\
  8  & 4 & < .001 s   \\
  10 & 5 & \sim 15.34 s \\
  12 & 6 & \sim 6 h \\         
  \hline             
  \end{array}
  \qquad
  %
  \begin{array}{|c|c|c|}
  \hline
  n  & k & \rm{time}    \\
  \hline
  4  & 2 & < .001 s  \\
  6  & 3 & < .001 s  \\
  8  & 4 & < .001 s    \\
  10 & 5 &  \sim 7.91 s   \\
  12 & 6 &  \sim 42 m        \\   
  \hline
  \end{array}
  \qquad
  %
  \begin{array}{|c|c|c|}
  \hline
  n  & k & \rm{time}    \\
  \hline
  4  & 2 & < .001 s  \\
  6  & 3 & < .001 s  \\
  8  & 4 & < .001 s \\
  10 & 5 & < .001 s   \\
  12 & 6 &   1.85 s \\        
  \hline
  \end{array}
$$

}

